State Representation Learning for Control: An Overview

Representation learning algorithms are designed to learn abstract features that characterize data. State representation learning (SRL) focuses on a particular kind of representation learning where learned features are in low dimension, evolve through time, and are influenced by actions of an agent. The representation is learned to capture the variation in the environment generated by the agent's actions; this kind of representation is particularly suitable for robotics and control scenarios. In particular, the low dimension characteristic of the representation helps to overcome the curse of dimensionality, provides easier interpretation and utilization by humans and can help improve performance and speed in policy learning algorithms such as reinforcement learning. This survey aims at covering the state-of-the-art on state representation learning in the most recent years. It reviews different SRL methods that involve interaction with the environment, their implementations and their applications in robotics control tasks (simulated or real). In particular, it highlights how generic learning objectives are differently exploited in the reviewed algorithms. Finally, it discusses evaluation methods to assess the representation learned and summarizes current and future lines of research.

==> graphes/Old_figures.tex <==

\begin{figure}
 
 \centering 
   \begin{subfigure}[b]{0.4\textwidth}
   \includegraphics[scale=0.2]{Images/Auto_Encoder_old.pdf}
   \caption{Auto-Encoder: reconstructing the observation. The error is computed between observation $o_t$ and its reconstruction $\hat{o}_t$}
   \label{fig:AutoEncoder}
 \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
   \includegraphics[scale=0.2]{Images/forward_model.pdf}
   \caption{Forward Model: predicting next state $s_{t+1}$ from $s_t$ and $a_t$. The error is computed between predicted state $\hat{s}_{t+1}$ and the actual next state $s_{t+1}$}
   \label{fig:ForwardModel}
 \end{subfigure}
 
 \begin{subfigure}[b]{0.4\textwidth}
   \includegraphics[scale=0.2]{Images/inverse_model.pdf}
   \caption{Inverse Model: predicting action $a_t$ from $s_t$ and $s_{t+1}$. The error is computed between predicted action $\hat{a}_t$ and the actual action $a_t$}
   \label{fig:InverseModel}
 \end{subfigure} 
  \begin{subfigure}[b]{0.4\textwidth}
   \includegraphics[scale=0.2]{Images/prior_model.pdf}
   \caption{Model with prior: The error is computed by applying loss functions on several states and action}
   \label{fig:Priors}
 \end{subfigure}
 
 \begin{subfigure}[b]{0.8\textwidth}
   \centering
   \includegraphics[scale=0.2]{Images/all_models.pdf}
   \caption{Example of hybrid model (E2C \cite{Watter15}) combining a set of previously described \textit{loss term blocks} in a-d. Several errors are used to learn the state representation using at the same time a forward model error, a reconstruction error and a constraint on the representation}  
   
   
   %Each associated loss function could optionally consider rewards $r_t$ (such as in some of the priors), or prediction errors including any combination of ${s_t, a_t, r_t, s_{t+1}, a_{t+1}, r_{t+1}}$} }
   \label{fig:AllModels}
 \end{subfigure}
   \caption{Illustration of the different objective functions used in SRL. $\tilde{s}_t$ represents the unknown true state, $s_t$ the learned state, and $\hat{s}_t$ the estimation or prediction of the learned state (similarly for observation $o$ and action $a$).  Each schema illustrates the variables that are exploited in the loss functions.}
\label{fig:models}
\end{figure}

==> removed_comment.tex <==


 %new Nat on learning disentangled representations NIPS workshop:
%  Based on the representation learning literature and the latest trends on learning disentangled representations \footnote{Learning Disentangled Representations: from Perception to Control NIPS Workshop: https://sites.google.com/view/disentanglenips2017}, we agree on the commonalities of disentangled representation learning as a common goal shared by the objectives of SRL:
%  \begin{itemize}
%  \item Learned representations must be sufficient, as efficient as possible (i.e., easy to work with, e.g., factorizing the data-generating factors), and minimal (from all possible representations, take the most efficient one). %N: can only have the poster, no paper in arxive yet for "Disentangling by factorizing" but I have poster picture
%  \item Like with learning disentangled representations, in SRL we are interested in unsupervised SRL.
%  \item Establishing a concrete task does not convert an unsupervised problem into a supervised one. %[as Bengio said at NIPS17] 
% \item Independence of features alone is not enough to provide a good quality of representations.
% \item L1 and L2 norms are meaningless proxy metrics as reconstruction error while we are discarding data away during representation learning. An open problem is finding better metrics.
% \item Representation learning will never provide more information than the initial one, and thus, only redundant information must be wisely discarded.
%  \item Features being linearly separable does not mean they are disentangled.
%  %\item Disentangling by factorizing is a novel trend (see workshop program)
%  \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% David : I don't see right now how to link this to the current paper content
% \subsubsection{Manifold learning}
% The observation space $\mathcal{O}$ can be seen as a manifold which holds all the observations, and $\mathcal{S}$ as a manifold of the representation. The goal is then to find a mapping between $\mathcal{O}$ and $\mathcal{S}$. We assume that a true $s_t \in \mathcal{S}$ exists. But $\mathcal{S}$ also holds all $s'_t$ such that it exists a bijection between $s_t$ and $s'_t$. In this survey, for the sake of simplicity, we will not use the manifold terminology and will only consider state and observation spaces.
% \subsubsection{Distribution learning}
% The observation space $\mathcal{O}$ can also be interpreted as a set of samples produced by a probability distribution $P(o_t|s_t)$ (with $s_t \in \mathcal{S}$) (\cite{Watter15,Assael15,Hoof16,Krishnan15,Karl16}. $\mathcal{S}$ is generated by another distribution $P(s)$. $\mathcal{S}$ is then the set of samples from $P(s_t)$. SRL is then the approximation of the probability distribution such as $P(s_t|o_t)$,  $P(s_t|s_{t-1},a_t)$ or $P(s_t|s_{t-1},s_{t-2})$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% David : I think it is not really useful to say all this
%\tim{i am not convinced by this part...}   What this paper is not:
%Given that we focus on robotics control applications of SRL in reinforcement learning (RL), this survey presents inverse models; however it does not consider approaches in inverse reinforcement learning, which do normally not learn a representation of states (inverse RL instead learns a reward function). It also focuses mainly on Markovian state spaces, although some time window approaches are also considered. We also touch upon some self-supervised methods; however, despite of the success of many recent autoregressive models, we do not expand on the latter because they do not learn a state space despite being self-supervised. Other end-to-end deep RL (DRL) approaches with the same objective as ours (robotics control) are also left out of the scope of this survey because we focus on SRL that can reuse learned states in transfer learning, e.g., for new domains, simulation-to-real or new tasks or scenarios.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{General evaluation techniques in representation learning }
%David :  I don't understand the link with Evaluating state representation ?-> Nat: it is general about representation learning evaluation, you are right.
%When it comes to providing a quantitative value that estimates the quality of a representation, in the context of representation learning, this can be harder than expected. The assessment should show if the representation we learned conforms to what we expect. While toolboxes to benchmark the robustness of machine learning models exists \cite{Rauber17}, understanding intermediate layers during the development of learning methods can be challenging. An approach in this direction is using linear classifier probes \cite{Alain16}, as well as using class-enhanced attentive responses \cite{Kumar17}. The latter enables the visualization of the activations for the most dominant classes.  Other way of assessing dimensionality reduction algorithms is in terms of their loss of quality \cite{Gracia14}, while adversarial methods can be tested with a suite of adversarial attacks \cite{Rauber17}. For instance, Foolbox\footnote{\url{https://pypi.python.org/pypi/foolbox}} creates adversarial examples that fool neural networks with gradient-based and black box attacks. % TODO could we cite a paper and not a slidedeck from On the Quantitative Evaluation of Deep Generative Models Russ Salakhutdinov*  [pdf](www.cs.cmu.edu/~rsalakhu/talk_Eval.pdf)?

%Linear classifier probe: We start from the concept of Shanon entropy, which is the classic way to describe the information contents of a random variable. We then seek to apply that concept to understand the roles of the intermediate layers of a neural network, to measure how much information is gained at every layer (answer : technically, none). We show that it fails to apply, and so we propose an alternative framework to ask the same question again.


%The deep reinforcement learning community has made available a large set of software benchmarks to test RL algorithms \cite{Arulkumaran17}. Despite the growing interest in making robotic applications work in real life settings, simulation environments are the de-facto start point and where most of the algorithms design, learning and evolution happen. Within the robotics domain, most used middleware is open-source: ROS, YARP, OROCOS, Player, etc. and some, also cross-platform \cite{Ivaldi14}. The top 7 most currently used simulators, in decreasing order, are Gazebo, ODE, Bullet, OpenRave, V-Rep, XDE, and Blender. Examples of most recently added RL Gym environments to PyBullet\footnote{\url{http://pybullet.org}} Minitaur quadruped, MIT race car, KUKA grasping, Ant, Hopper, Humanoid etc. These simulation environments are mainly designed for RL, but they could equally be used to test state representation algorithms.

%While the broad choice allows roboticists to pick the best middleware for their needs, it also makes comparing AI models very challenging, since dynamics models and simulators' performance comparison easily introduces noise, calibration issues and instabilities that are susceptible of making the algorithms sensible to them. Reproducibility also becomes compromised.

%Despite the above being the best softwares upon users ratings \cite{Ivaldi14}, the challenge of not having reproducible datasets for robotics both in simulation and real live makes these simulators practically unusable as platforms to support research benchmarks. This is why most research builds on RL toy tasks or the more broad set of Atari 2600 video games from the Arcade Learning Environment (ALE) \cite{Bellemare13,Machado17}. However, the further development of similar standard datasets and benchmarks for robotic control tasks is a crucial gap yet to be filled.

%Examples of challenging games that involve further planning and strategic thinking in the near future include \textit{Freeway} and \textit{Montezuma's revenge}. \textit{Freeway} is a game in which a chicken is expected to cross the road while avoiding cars, well suited to observe options in which the agent clearly wants to reach a specific lane in the street, %a histogram representing the chicken’s height during an episode is used for evaluation We can clearly see how the chicken’s height varies for different
%since a random walk over primitive actions does not explore the environment properly as shown in \cite{Machado17a}. %Remarkably, option #445 scores 28 points at the end of the episode, without ever explicitly taking the reward signal into consideration. This performance is very close to those obtained by state-of-the-art algorithms.
%In Montezuma's revenge, the objective is to navigate a room to pickup a key to open a door, and thus, option discovery and valuation is key (see \cite{Kulkarni16} and \cite{Machado17a}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
